Large Language Models for Software Testing Education: an Experience Report

The rapid integration of Large Language Models (LLMs) into software engineering practice is reshaping how software testing activities are performed. LLMs are increasingly used to support software testing. Consequently, software testing education must evolve to prepare students for this new paradigm. However, while students have already begun to use LLMs in an ad hoc manner for testing tasks, there is limited empirical understanding of how such usage influences their testing behaviors, judgment, and learning outcomes. It is necessary to conduct a systematic investigation into how students learn to evaluate, control, and refine LLM-assisted testing results. This paper presents a mixed-methods, two-phase exploratory study on human-LLM collaboration in software testing education. In Phase I, we analyze classroom learning artifacts and interaction records from 15 students, together with a large-scale survey conducted in a national software testing competition (337 valid responses), to identify recurring prompt-related difficulties across testing tasks. The results reveal systematic interaction breakdowns, including missing contextual information, insufficient constraints, rigid one-shot prompting, and limited strategy-driven iteration, with automated test script generation emerging as a particularly heterogeneous and effort-intensive interaction context. Building on these findings, Phase II conducts an illustrative classroom practice that operationalizes the observed breakdowns into a lightweight, stage-aware prompt scaffold for test script generation, guiding students to explicitly articulate execution-relevant information such as environmental assumptions, interaction grounding, synchronization, and validation intent, and reporting descriptive shifts in students' testing-related articulation when interacting with LLMs.

==> tables/RQ2table2.tex <==
\begin{table*}
\centering
\caption{Questions and answers of questionnaire about LLM}
\label{rq2table2}
\small % 或 \small，根据需要
\begin{tblr}{
  vline{2} = {-}{},
  hline{1-7} = {-}{},
  colspec = {X[1,l] X[2,l]}, % 问题列占1份，答案列占2份
  row{1} = {font=\bfseries},
}
  Question
                                                                   & 
  Answer
                   \\
 In which aspects does the LLM facilitate the requirement analysis phase?
                                                   & 
  Improve analysis efficiency; extract key information; image recognition and requirement matching; generate functional requirement documents; assist test requirement writing and functional requirement supplement.~~ 
             \\
In what specific areas does the LLM assist during the test requirement generation phase?
                                                 & 
  Generate requirement documents; generate test requirement tables; generate preliminary test requirements; analyze and split test requirement points; generate test points and flow charts to ensure the comprehensiveness of test requirements.
     \\
What challenges were encountered when utilizing LLMs for test case generation, and what could be the underlying reasons for these challenges?
                 & 
In the test case generation phase, the following issues were encountered with LLMs: some test cases included non-functional requirements; the overall coverage of the test cases did not meet the expected standards; the detailed descriptions of the test cases were insufficient, affecting the testing effectiveness; the model struggled to output all relevant test cases in one round when involving multiple test points; there were difficulties in understanding complex business logic; the generation process of test cases often resulted in incomplete cases; incorrect filling of environmental configuration data was also a common problem. "
                                                                                                        \\
What are your insights into why the generated test scripts are not immediately executable? What supplementary information should be furnished to the large language model to enhance its ability to generate test scripts effectively?

   & 

In the test script generation phase, the main reasons why the scripts are not directly executable involve several aspects: logical errors exist within the scripts; the generated code is incompatible with the required dependency libraries; the page element locators are not accurate enough; the scripts lack an effective exception handling mechanism; the element locators and driving methods used are not flexible enough; appropriate assertion methods are not utilized. 
  
To improve the quality of test scripts generated by the LLM, the following additional information should be provided: detailed test requirements and business logic descriptions, specific details of the runtime environment (including operating system type, software version numbers, dependency library versions, etc.), precise page element locator information, clear exception handling procedures, correct element locator strategies, detailed user operation steps and corresponding judgment conditions, specific location information of interactive elements, as well as hints and suggestions for deprecated libraries and their alternatives.
                                          \\
What are the common issues that occur when employing a large language model to produce test scripts?
                                           & 

During the process of using a LLm to generate test scripts, several key issues encountered: Firstly, incompatibilities in environment configuration prevent the scripts from being executed directly; secondly, the scripts fail to cover all necessary test functionality; thirdly, there are accuracy issues with element location, and the methods used may not be applicable or require manual supplementation; additionally, the script structure is complex and contains unnecessary redundant steps; there is insufficient capability in handling dynamic content; there is a discrepancy with the conventional thinking patterns of testers; there are difficulties in understanding complex business processes; the scripts have poor readability and maintainability; the test coverage does not meet expectations; there are issues with fixed wait times and hard-coded problems; and there is a lack of understanding of context as well as a deficiency in creativity and flexibility. To address these issues, we need to provide more detailed prompts to ensure that LLMs can generate high-quality test scripts that align with actual requirements, can be executed directly, and are easy to maintain subsequently.
   
\end{tblr}
\end{table*}

==> tables/likert_classroom.tex <==



\begin{table*}
\centering
\caption{Classroom-only Likert responses (raw matrix) and item-level summary statistics ($N=15$).
Scale: 1 = strongly disagree, 5 = strongly agree.}
\label{tab:classroom-likert-matrix}
\resizebox{\linewidth}{!}{
\begin{tblr}{
  vline{2,17} = {-}{},
  hline{1-2,7} = {-}{},
  cell{1}{2} = {c=15}{},
  colspec = {
    Q[l, leftsep=4pt, rightsep=4pt]        % Questions 列，稍宽松保证可读
    *{15}{Q[c, leftsep=2pt, rightsep=2pt]} % 15个学生打分列，紧凑
    *{3}{Q[c, leftsep=4pt, rightsep=4pt]}  % Total, AVG, Var，稍比学生列宽松一点，提升可读性
  },
}
Questions       & Students  &   &   &   &   &   &   &   &   &   &   &   &   &   &   & Total   & AVG  & Var  \\
The requirements analysis task can be left entirely to the LLM.     & 5 & 4 & 4 & 3 & 3 & 3 & 3 & 4 & 4 & 3 & 4 & 4 & 3 & 3 & 3 & 53.0 & 3.5 & 0.4 \\
The task of test requirements generation can be left entirely to the LLM.   & 4 & 4 & 4 & 4 & 3 & 3 & 2 & 4 & 4 & 3 & 4 & 4 & 2 & 3 & 3 & 51.0 & 3.4 & 0.5 \\
The test case generation can be left entirely to the LLM.   & 4 & 4 & 3 & 3 & 3 & 3 & 3 & 4 & 4 & 2 & 4 & 4 & 1 & 4 & 3 & 49.0 & 3.3 & 0.7 \\
The test scripts generation can be left entirely to the LLM.    & 5 & 4 & 3 & 3 & 3 & 3 & 3 & 4 & 4 & 2 & 4 & 3 & 1 & 4 & 4 & 50.0 & 3.3 & 0.9 \\
LLMs are sufficiently helpful during the test report generation phase. & 5 & 5 & 3 & 4 & 4 & 3 & 3 & 5 & 4 & 4 & 4 & 4 & 4 & 4 & 3 & 59.0 & 3.9 & 0.5 
\end{tblr}}
\vspace{-4mm}
\end{table*}

==> tables/likert_items.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\caption{Perceived efficiency gains from LLM assistance (Q4, valid responses $N=337$).
Scale: 1 = almost no improvement, 5 = significant improvement.}
\label{tab:survey-q4}
\begin{tabular}{@{} p{6.3cm} c c c c c c c @{}}
\toprule
\textbf{Item} & \textbf{N} & \textbf{Mean (SD)} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} \\
\midrule
Test case design efficiency: quickly generating test steps and expected results
& 337 & 3.664 (0.982) & 2.36\% & 9.73\% & 27.14\% & 40.71\% & 20.06\% \\
Test script writing efficiency: generating code structures (e.g., XPath locators, action logic)
& 337 & 3.319 (1.065) & 6.49\% & 13.27\% & 35.10\% & 32.15\% & 12.98\% \\
Test planning efficiency: defining test scope, priorities, and automation coverage strategy
& 337 & 3.499 (0.998) & 3.83\% & 10.62\% & 32.45\% & 38.05\% & 15.04\% \\
Test evaluation efficiency: assisting report generation and failure analysis (e.g., root-cause localization, risk summary)
& 337 & 3.481 (1.019) & 4.72\% & 10.62\% & 30.97\% & 39.23\% & 14.45\% \\
Overall testing efficiency: end-to-end improvement across design, scripting, and execution
& 337 & 3.563 (0.966) & 3.24\% & 8.85\% & 31.86\% & 40.41\% & 15.63\% \\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\caption{Perceived impact of prompt-related issues on test script generation outcomes
(Q8, valid responses $N=337$).
Scale: 1 = no impact, 5 = directly leads to failure.}
\label{tab:survey-q8}
\begin{tabular}{@{} p{6.3cm} c c c c c c c @{}}
\toprule
\textbf{Item} & \textbf{N} & \textbf{Mean (SD)} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} \\
\midrule
Task description too vague (e.g., only saying ``write a login test'')
& 337 & 3.457 (0.864) & 2.36\% & 8.26\% & 40.12\% & 39.82\% & 9.44\% \\
Missing context (e.g., requirements / UI / environment)
& 337 & 3.451 (0.825) & 1.47\% & 7.96\% & 43.66\% & 37.76\% & 9.14\% \\
Not iteratively refining the output via follow-up questions
& 337 & 3.301 (0.824) & 2.36\% & 9.73\% & 49.85\% & 31.56\% & 6.49\% \\
Not specifying constraints (framework / language / output format)
& 337 & 3.322 (0.874) & 3.54\% & 8.55\% & 48.08\% & 31.86\% & 7.96\% \\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\caption{Concerns about over-reliance on LLMs and perceived learning impact
(Q9, valid responses $N=337$).
Scale: 1 = strongly disagree, 5 = strongly agree.}
\label{tab:survey-q9}
\begin{tabular}{@{} p{6.3cm} c c c c c c c @{}}
\toprule
\textbf{Item} & \textbf{N} & \textbf{Mean (SD)} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} \\
\midrule
Over-reliance on LLMs may reduce my test design ability
& 337 & 3.295 (0.989) & 3.24\% & 19.47\% & 30.97\% & 37.17\% & 9.14\% \\
Over-reliance on LLMs may reduce my test case writing ability
& 337 & 3.319 (0.966) & 2.65\% & 19.17\% & 30.38\% & 39.23\% & 8.55\% \\
Over-reliance on LLMs may reduce my test scripting ability
& 337 & 3.322 (0.997) & 4.13\% & 16.81\% & 31.27\% & 38.35\% & 9.44\% \\
Over-reliance on LLMs may reduce my competitiveness in employment
& 337 & 3.118 (1.019) & 5.60\% & 22.42\% & 33.92\% & 30.68\% & 7.37\% \\
\bottomrule
\end{tabular}
\end{table*}

